HAVAPlot: A Web-Based Scientific Visualization and Post-Processing Platform

This paper presents HAVAPlot, a browser-based framework for scientific visualization and post-processing of numerical simulation data. Operating entirely within the user's browser, HAVAPlot requires no software installation or data uploads while supporting mesh-based and tabular datasets beyond computational fluid dynamics. The framework directly reads native OpenFOAM cases, including polyhedral meshes, ASCII and binary fields, boundary data, and Lagrangian particles, as well as legacy and XML VTK files and tabular datasets. It provides line, contour, and three-dimensional plots; exact polyhedral slicing; boundary extraction; variable calculations; customizable color scales; symmetry mirroring; zoomed insets; streamlines; isosurfaces; particle visualization; and vector PDF/EPS and data export. The underlying numerical algorithms are independently verified. Cell centers and volumes agree with an independent implementation of OpenFOAM's geometric algorithm, while 6.1 million field values across four two-dimensional, axisymmetric, and three-dimensional production cases are reproduced to machine precision. For analytical fields on distorted hexahedral meshes, cell-to-point interpolation exhibits second-order convergence in the interior and first-order convergence at boundaries. Meshes containing 250,000 cells load in at most 1.3 seconds. Applications to an impinging supersonic jet, hypersonic cylinder flow, a hybrid particle-continuum cold-spray nozzle, a three-dimensional gas-bearing film, and supersonic cone flow demonstrate the framework's capabilities.

==> data/perf_table.tex <==
2D & 1{,}024 & 4{,}160 & 38 & 9.09 & 71 & 35 & -- \\
2D & 4{,}096 & 16{,}512 & 57 & 3.43 & 74 & 40 & -- \\
2D & 16{,}384 & 65{,}792 & 119 & 1.81 & 65 & 50 & -- \\
2D & 65{,}536 & 262{,}656 & 361 & 1.37 & 196 & 146 & -- \\
2D & 262{,}144 & 1{,}049{,}600 & 1337 & 1.27 & 359 & 305 & -- \\
3D & 13{,}824 & 43{,}200 & 84 & 1.95 & 111 & 102 & 420 \\
3D & 32{,}768 & 101{,}376 & 157 & 1.55 & 75 & 61 & 239 \\
3D & 110{,}592 & 338{,}688 & 394 & 1.16 & 45 & 42 & 123 \\
3D & 262{,}144 & 798{,}720 & 843 & 1.06 & 85 & 82 & 198 \\


==> data/reader_table.tex <==
Cold-spray nozzle (axisym.) & \texttt{uniGasHAVAMPPICFoam} & 24{,}980 & 65 & 1{,}623{,}700 & 268 & $8.1\times10^{-13}$ & $4.5\times10^{-14}$ & $4.4\times10^{-16}$ & $1.8\times10^{-1}$ \\
Impinging jet (axisym.) & \texttt{rhoCentralFoam} & 68{,}123 & 17 & 1{,}158{,}091 & 285 & $1.5\times10^{-13}$ & $8.9\times10^{-14}$ & $4.4\times10^{-16}$ & $7.9\times10^{-2}$ \\
HEG cylinder (2D) & \texttt{hy2Foam} & 62{,}001 & 33 & 2{,}046{,}033 & 433 & $3.0\times10^{-13}$ & $2.8\times10^{-12}$ & $3.9\times10^{-16}$ & $8.9\times10^{-4}$ \\
Bearing film (3D) & \texttt{rhoSimpleFoam} & 157{,}080 & 8 & 1{,}256{,}640 & 382 & $2.8\times10^{-13}$ & $6.2\times10^{-14}$ & $4.1\times10^{-16}$ & $1.9\times10^{-3}$ \\

